Routing Optimization Based on Distributed Intelligent Network Softwarization for the Internet of Things

The Internet of Things (IoT) establishes connectivity between billions of heterogeneous devices that provide a variety of essential everyday services. The IoT faces several challenges, including energy efficiency and scalability, that require consideration of enabling technologies such as network softwarization. This technology is an appropriate solution for IoT, leveraging Software Defined Networking (SDN) and Network Function Virtualization (NFV) as two main techniques, especially when combined with Machine Learning (ML). Although many efforts have been made to optimize routing in softwarized IoT, the existing solutions do not take advantage of distributed intelligence. In this paper, we propose to optimize routing in softwarized IoT networks using Federated Deep Reinforcement Learning (FDRL), where distributed network softwarization and intelligence (i.e., FDRL) join forces to improve routing in constrained IoT networks. Our proposal introduces the combination of two novelties (i.e., distributed controller design and intelligent routing) to meet the IoT requirements (mainly performance and energy efficiency). The simulation results confirm the effectiveness of our proposal compared to the conventional counterparts.

==> algorithm1.tex <==
\begin{algorithm}[!h]
 \caption{FDRL Aggregator Training Algorithm}
 \label{algo:agg}
 \SetKwInOut{Input}{Inputs}
 \SetKwInOut{Output}{Output}
 \Input{$R$ : Number of rounds\\
$W$ : Number of learning nodes\\}
\Output{$\theta^*$ : Global model weights}

send initial weights $\theta^0$ to learning nodes

\For{$r\gets 1$ \KwTo $R$ }{
\For{$w\gets 1$ \KwTo $W$ }{
wait for $\theta^{w,r}$
}
$\theta^r\gets \frac{1}{W}\sum_{w=1}^{W}\theta^{w,r}$

send updated weights $\theta^r$ to learning nodes
			 
}
 $\theta^* \gets \theta^r$
\end{algorithm}

==> algorithm2.tex <==
\begin{algorithm}[!h]
 \caption{FDRL Learning Node Training Algorithm}
 \label{algo:work}
 \SetKwInOut{Input}{Inputs}
 \SetKwInOut{Output}{Output}
 \Input{$A_g$ : Aggregation period\\
 $N_e$ : Number of training episodes\\
 $T$ : Episode horizon time\\
 $\epsilon$ : Exploration parameter\\}
\Output{$\theta^*$ : Global model weights}

wait for initial global weights $\theta^g$ from aggregator

\For{$e\gets 1$ \KwTo $N_e$ }{

$\theta^e\gets \theta^g$

get current state \(s_t\)

\For{$t\gets 1$ \KwTo $T$ }{

generate a random number \(\rho\in [0,1]\)

$a_t\gets$
\begin{cases}
  \text{pick an action that maximizes $U(t)$} & \text{if $\rho>\epsilon$} \\
  \text{pick a random action $a\in A$} & \text{else}
\end{cases}

take action $a_t$ to go to state $s_{t+1}$ and get reward $r_{t+1}$

store $\{$s_t$, $a_t$, $s_{t+1}$, $r_{t+1}$\}$

}

update $\theta^e$

\If{\textsf{$e\mod A_g = 0$}}
{

send $\theta^e$ to the aggregator

wait for the aggregated value $\theta^g$

}			 
}

$\theta^* \gets \theta^g$

\end{algorithm}
